Can One Embedding Fit All? A Multi-Interest Learning Paradigm Towards Improving User Interest Diversity Fairness

Recommender systems (RSs) have gained widespread applications across various domains owing to the superior ability to capture users' interests. However, the complexity and nuanced nature of users' interests, which span a wide range of diversity, pose a significant challenge in delivering fair recommendations. In practice, user preferences vary significantly; some users show a clear preference toward certain item categories, while others have a broad interest in diverse ones. Even though it is expected that all users should receive high-quality recommendations, the effectiveness of RSs in catering to this disparate interest diversity remains under-explored. In this work, we investigate whether users with varied levels of interest diversity are treated fairly. Our empirical experiments reveal an inherent disparity: users with broader interests often receive lower-quality recommendations. To mitigate this, we propose a multi-interest framework that uses multiple (virtual) interest embeddings rather than single ones to represent users. Specifically, the framework consists of stacked multi-interest representation layers, which include an interest embedding generator that derives virtual interests from shared parameters, and a center embedding aggregator that facilitates multi-hop aggregation. Experiments demonstrate the effectiveness of the framework in achieving better trade-off between fairness and utility across various datasets and backbones.

==> model.tex <==
\section{The Proposed Multi-Interest Model}
\label{sec:model}

% Based on the observation in Sec.~\ref{sec:preliminary} that current RS models are insufficient to match user and item embeddings for user with diverse interests which results in the recommendation disparity among user groups with various levels of interest diversity,
To mitigate the unfairness observed in Sec.~\ref{sec:preliminary}, we dive into the potential reason causing such disparity from the perspective of embedding space, which motivate us to propose a multi-interest framework where each user is represented by multiple embeddings. These embeddings learn a better representation for users' interests and thus benefit the performance of user with high interest diversity. In this way, the unfairness is mitigated by maintaining the performance for users from low interest diversity group and improving the performance for users form high interest diversity group.

In the following, we first discuss the potential reason in Sec.~\ref{sec.motivation}, and give an overview of the multi-interest framework in Sec.~\ref{sec.overview} and elaborate the detailed components in Sec.~\ref{sec.component} along with the optimization in Sec.~\ref{sec.opt}.

\subsection{Motivation: Discussion of Potential Reasons}
\label{sec.motivation}
% \yy{move this part to the model section as the motivation}
% \yy{some insights and potential discussions of why this happens which could better motivate the following: e.g., alignment of different groups, can also include the collaborative filtering effect as another potential reason and we leave it as future work (but this could potentially shift the paper attention)}

Since the core component in RS is to learn high-quality user and item embeddings, we investigate the potential reasons from the embedding space. Prior research has underscored the correlation between embedding alignment (i.e., the capacity to bring users and their associated items into proximity) and utility performance~\cite{wang2022towards,wang2020understanding}. A superior alignment typically correlates with enhanced performance.
% Existing researches have identified the closeness between embedding alignment (i.e., the ability of bringing user and their interacted items together) and utility performance~\cite{wang2022towards,wang2020understanding} where a better alignment would contribute to a better performance. 
The alignment definition is as follows:
\begin{align}
    {\text{alignment}} = \mathbb{E}_{(u,i) \sim p_{\text{pos}}} \left\| \tilde{\mathbf{e}_u} - \tilde{\mathbf{e}_i} \right\|^2,
\end{align}
where $\tilde{\mathbf{e}_u}$ and $\tilde{\mathbf{e}_i}$ are the $l_2$ normalized user and item representations from historical interacted pairs. It measures the distance in the unit hypersphere and the lower the better. To uncover the potential reason for disparity among groups, rather than calculating the overall alignment, we measure the alignment in a group level. Results in Fig.~\ref{fig:preliminary_alignment} (results for other datasets are included in Appedix~\ref{app:preliminary}) show that (1) CAGCN$^*$ exhibits superior alignment compared to LightGCN, a consistency mirrored in the performance illustrated in Fig.~\ref{fig:preliminary}; (2) Users displaying a broader spectrum of interests tend to have less optimal alignment within the embedding space. This suggests that the current framework might not be adequately efficient in aligning users and items, particularly when users have a wide array of interests.
% Users with higher interest diversity have a poorer alignment in the embedding space, indicating the current framework's insufficiency in aligning user and item well, especially for user with diverse interests.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.48\textwidth]{figure/preliminary_alignment.png}
    \caption{Group embedding alignment of ml-1m dataset based on \textcolor{orange}{LightGCN} and \textcolor{blue}{CAGCN$^*$}.}
    \label{fig:preliminary_alignment}
\end{figure}

This observation is closely related to multi-interest research~\cite{zhang2022re4,li2019multi} which assumes that single embedding is insufficient to capture the characteristics. As shown in Fig.~\ref{fig:motivation}, since users' interests are diverse, the single embedding is insufficient to capture the interests: to maintain a close relationship with all interacted items, the learned single user embedding might fall in between which is not close to any of the real interests, resulting in low alignment. The recommended items based on this embedding thus become inaccurate. In contrast, when a user has multiple embeddings, for different items, the matching interest can be automatically obtained and corresponding recommendations will be made, leading to a more accurate interest modeling and recommendation. 

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.45\textwidth]{figure/motivation.png}
    \caption{Multi-interest motivation: single embedding is insufficient to capture users' interests.}
    \label{fig:motivation}
\end{figure}


\subsection{Model Architecture}
\label{sec.overview}

\begin{figure*}[htbp]
    \centering
    \includegraphics[width=0.95\textwidth]{figure/framwork.png}
    \caption{Multi-interest framework: rather than a single embedding, each user/item is represented by multiple embeddings (Interest number equals two in this example).}
    \label{fig:framework}
\end{figure*}


Fig.~\ref{fig:framework} shows the multi-interest framework where each user/item has different types of embeddings, including (1) center embedding $\mathbf{E}_C^l \in \mathbb{R}^{N\times d}$ representing users/items main characteristic/features where $N$ is the number of node (including users and items) and $d$ is the dimension; (2) virtual embedding $\mathbf{E}_V^l \in \mathbb{R}^{N\times K\times d}$ which relate to specific interests where $K$ is the number of interests; (3) total embedding $\mathbf{E}_T^l \in \mathbb{R}^{N\times K\times d}$ which is a weighted summation of center and virtual embedding (i.e., $\mathbf{E}_T^l[v_i, k] = \mathbf{E}_C^l[v_i] + \lambda \mathbf{E}_V^l[v_i, k]$), providing a comprehensive view about the main characteristic along with interests. Among these embeddings, center embeddings are learnable parameters while the other two types of embeddings are calculated based on center embeddings with the multi-interest extractor. This mechanism avoids introducing too many learnable parameters by sharing the global interest parameter in the attention mechanism.

With these notations, the framework is as follows: (1) Given the user-item graph, user and item embeddings are obtained after performing the multi-interest representation layer which will be introduced in the next subsection. (2) After obtaining the embeddings, the relevance score for user, item pair $(v_u, v_i)$ is calculated as 
\begin{equation}
    \hat{y}_{ui}=\max_{k=1}^K \mathbf{E}_T[v_u, k]^\top \mathbf{E}_C[v_i].
    \label{eq.relevance}
\end{equation}
(3) These predicted relevance scores are optimized along with the ground truth in Bayesian Personalized Ranking Loss (BPR) loss~\cite{rendle2012bpr} $\mathcal{L}_{\text{BPR}}$ while an independence loss $\mathcal{L}_{\text{IND}}$ is designed to encourage the model to learn diverse global interests.


\subsection{Multi-Interest Representation Layer}
\label{sec.component}
In this section, we introduce the details about the multi-interest representation layer which is designed to learn high-quality center/virtual/total representations. This layer first generates the total embeddings based on the interactions and the center embeddings are updated during aggregation. Layers can be stacked to allow multi-hop aggregations.

\textbf{Total embedding generation:} Total embedding is the summation of center and virtual embeddings. Virtual embeddings of $l$-th layer for node $v_i$ and aspect $k$ is calculated as the weighted average of the center embeddings of neighbors where the weight is calculated in Eq.~\ref{eq.att} based on attention mechanism where $T$ is the temperature to control the smoothness of attentions. The attentions are based on the similarity with global interests denoted as $\mathbf{w}_k^l$. For $k$-th aspect, if an item is closely related to this aspect, the attention will be high, leading to a larger aggregation from this item. Therefore, total embedding $\mathbf{E}_V^l[v_i, k]$ captures information related to $k$-th aspect.
\begin{equation}
    \mathbf{E}_V^l[v_i, k] = \sum_{v_j \in \mathcal{N}_{v_i}}a_{k, v_j}^l \mathbf{E}_C^l[v_j]
\end{equation}

\begin{equation}
    a_{k, v_i}^l = \frac{\text{exp}(\text{cos}(\mathbf{E}_C[v_i]^l, \mathbf{w}_k^l)/T)}{\sum_{j} \text{exp}(\text{cos}(\mathbf{E}_C[v_i]^l, \mathbf{w}_j^l)/T)}
    \label{eq.att}
\end{equation}

Note that this component currently is based on simple attention mechanism but can be further substituted with more advanced generative methods to generate total embeddings representing both main characteristic and interest perspectives.

\textbf{Center embedding aggregation:} Neighborhood information provide additional information about each node. Therefore, we design a multi-interest based aggregation which is similar to the LightGCN aggregation with the difference in the aggregated embeddings. Since the other two types of embeddings are based on center embeddings, we only update center embeddings during aggregation. We have the aggregation process as follows

\begin{equation}
    \mathbf{E}_C^{l+1} = \mathbf{D}^{-0.5}\mathbf{A}\mathbf{D}^{-0.5} {\mathbf{E}_T^l}^\prime,
\end{equation}
where $\mathbf{D}$ is the diagonal degree matrix and $\mathbf{A}$ is the adjacency matrix.

Center embeddings $\mathbf{E}_C^{l+1}$ is updated based on total embeddings ${\mathbf{E}_T^l}$ where ${\mathbf{E}_T^l}^\prime$ is the matching slide among $K$ aspects as shown in Fig.~\ref{fig:framework}. The matching slides are selected from $K$ slides (i.e., $K$ total embeddings) if they have the maximum dot products with the center embedding. In this way, only necessary information from users and items is aggregated.


\subsection{Optimization}
\label{sec.opt}
We jointly utilize the BPR loss~\cite{rendle2012bpr} ($\mathcal{L}_{\text{BPR}}$) and independence loss ($\mathcal{L}_{\text{IND}}$)~\cite{du2023towards} to train our multi-interest RS.

\begin{equation}
    \mathcal{L}_{\text{BPR}} = -\sum_{(u, i, j) \in \mathcal{D}}\log\sigma(\hat{y}_{ui}-\hat{y}_{uj})+\lambda_{\Theta}\|\Theta\|^2,\label{eq.bpr}
\end{equation}
where $\mathcal{D}=\{(u,i,j)|u\in\mathcal{U}\land i\in \mathcal{I}_u^+\land j\in \mathcal{I}_u^-\}$ is the training dataset where $\mathcal{U}$ is the total user set, $\mathcal{I}_u^+$/$\mathcal{I}_u^-$ are the user sets that $u$ has/hasn't interacted with. $\sigma(\cdot)$ is sigmoid function, and $\Theta$ denoted the model parameter with $\lambda_{\Theta}$ controlling the $L_2$ norm to prevent over-fitting.
$\hat{y}_{ui}$ is the predicted preference/relevance score computed based on Eq.~\ref{eq.relevance}. 

Independence loss is introduced to encourage the learned global interests to be diverse from each other~\cite{du2023towards}.
\begin{equation}
    \mathcal{L}_{\text{IND}} = \sum_{k}-\text{log}\frac{\text{exp}(\text{cos}(\mathbf{w}_k, \mathbf{w}_k))}{\sum_{k^\prime} \text{exp}(\text{cos}(\mathbf{w}_k, \mathbf{w}_k^\prime))}
\end{equation}
This loss is based on mutual information for simplicity. Other methods such as distance correlation~\cite{szekely2007measuring}, orthogonality~\cite{liu2019hi} can also be used for modeling the independence.

The final loss is the summation of these two loss terms with coefficient $\lambda_{\text{IND}}$.
\begin{equation}
    \mathcal{L} = \mathcal{L}_{\text{BPR}}+\lambda_{\text{IND}} \mathcal{L}_{\text{IND}}
\end{equation}
